A Two-Phase Dynamic Throughput Optimization Model for Big Data Transfers

The amount of data moved over dedicated and non-dedicated network links increases much faster than the increase in the network capacity, but the current solutions fail to guarantee even the promised achievable transfer throughputs. In this paper, we propose a novel dynamic throughput optimization model based on mathematical modeling with offline knowledge discovery/analysis and adaptive online decision making. In offline analysis, we mine historical transfer logs to perform knowledge discovery about the transfer characteristics. Online phase uses the discovered knowledge from the offline analysis along with real-time investigation of the network condition to optimize the protocol parameters. As real-time investigation is expensive and provides partial knowledge about the current network status, our model uses historical knowledge about the network and data to reduce the real-time investigation overhead while ensuring near optimal throughput for each transfer. Our novel approach is tested over different networks with different datasets and outperformed its closest competitor by 1.7x and the default case by 5x. It also achieved up to 93% accuracy compared with the optimal achievable throughput possible on those networks.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> section-distributedapproach.tex <==

%\subsubsection{Distributed Approach}

\begin{figure}[t]
\centering
\includegraphics[keepaspectratio=true,angle=0,width=85mm]{figures/distributed_model.pdf}
\vspace{-3mm}
\caption{Overview of proposed optimization model} \label{fig:model_overview}
\end{figure}

In a distributed approach, each user tries to maximize their throughput without hurting other contending transfers. 
%
Here users are unaware of the characteristics of the other contending transfers. 
%
Therefore, each user needs to check the available bandwidth to set the parameters. 
%
Moreover, the user needs a mechanism to tune the parameters and ensure fairness constraint dynamically. 
%
At first, we describe the simplest solution for the distributed approach and explain its inefficiencies. 
%
In this solution, each user starts the transfer with default parameter values. 
%
Then periodically, the user increases the protocol parameters with constant steps until it detects queuing delay. 
%
Increasing queuing delay indicates upcoming congestion. 
%
Therefore, the user can cut back the parameter values up to a certain level. 
%
In case of packet loss (indicate congestion), the user reduces parameter values more drastically. 
%
We identify three major performance issues in this simple solution. 

(1) Protocol parameters are heavily dependent on end systems, network links, type of data, and application that performs data transfer. 
%
Different transfers need different protocol parameters to achieve optimal performance. 
%
Initial default parameter values could become sub-optimal at the beginning of the transfer. 
%
Therefore, we need an approach that can provide protocol parameters to individual transfers in a more personalized way. 

(2) The periodic additive increase of protocol parameters during the transfer could introduce extra overhead. 
%
When initial parameter choices are far away from optimal parameters, the transfer takes a longer time to reach the optimal parameter level. 
%
Moreover, the increase in concurrency/parallelism opens new TCP streams that go through TCP slow start phase. 
%
Therefore, we need an approach where protocol parameters can converge towards optimal level faster. 

(3) During congestion, the user reduces the parameters up to a predefined level. Too aggressive reduction of parameters can reduce performance. 
%
When congestion is over, transfer needs a longer time to reach the optimal level again.
% 
Therefore, we need a mechanism to reduce parameters up to a level that is good enough to clear congestion and close enough to optimal level. 
%
This strategy helps to regain optimal performance when congestion resolved. 

To resolve the issue (1) we need to access the impact of different protocol parameters 

\subsubsection{Centralized Approach}

\begin{figure}[t]
\centering
\includegraphics[keepaspectratio=true,angle=0,width=85mm]{figures/centralized_model.pdf}
\vspace{-3mm}
\caption{Overview of the distributed approach} \label{fig:distributed_model}
\end{figure}


In a centralized approach, a centralized traffic engineering module can schedule the transfers with adequately optimized parameters. The centralized module has access to overall network view. Therefore, it can precisely allocate protocol parameters to the contending transfers. During the network failures, it can precisely scale down or reroute the transfers without compromising the fairness constraint. It also can reallocate parameters when a transfer finishes or aborts. 
%However, it is not scalable in a very large scale system.
 
Given a source endpoint $e_s$ and destination endpoint $e_d$ with a link bandwidth $b$ and round trip time $rtt$; a dataset with a total size $f_{all}$, average file size $f_{avg}$,and  number of files $n$; and set of protocol parameters $\theta=\{cc, p, pp\}$, the throughput $th$ optimization problem can be defined as:

\begin{equation}
\begin{array}{ll}
\underset{ \{cc,p,pp\} }{\mathrm{argmax}} &  \displaystyle\int_{t_s}^{t_f} th(e_s,e_d,b,rtt,f_{avg}, n,cc,p,pp,l_{ctd}) \\
\text{subject to.} & cc \times p \leq \mathbb{N}_{streams} \\ 
				   & pp \leq \mathbb{P} \\
\end{array}
\end{equation}

where $t_s$ and $t_f$ are the transfer start and end times respectively. 
%As we are optimizing throughput function in a shared environment, other concurrent transfers can affect the behavior of achievable throughput. 
%We can account the incoming and outgoing transfers happening from the source and destination nodes. Our historical logs contain information of such transfers. 
We define the load from contending transfers as $l_{ctd}$. 

\begin{comment}
We have made some assumptions when defining our model, which are expressed below. 
%\newtheorem{assumption}{Assumption}
%\begin{assumption}\label{as:1}
 %Competing Transfers can achieve aggregate throughput, $T = \sum_{i=1}^{N} th_i$, where $N$ is the number of TCP streams for all competing transfers, and $th_i$ is the throughput of individual transfer $i$. 
When $u$ number of users are transferring, the aggregate throughput can be defined as, 
\begin{equation}
T = \sum_{i=1}^{\mathbb{U}} th_i, \quad \text{where} \quad \mathbb{U} = u \times cc \times p
\end{equation}
Where $\mathbb{U}$ is the number of streams for all competing transfers and $th_i$ is the achieved throughput for each stream. 
%\end{assumption}

%\begin{assumption}\label{as:2}
 After explaining the effect of known competing transfers, the fluctuation on transfer behavior depends on the intensity of the external load $l_{ext}$.  
%\end{assumption}

%\begin{assumption}\label{as:3}
For disk to disk transfer, Maximum achievable throughput, $th_{max}$ can be bounded by the end-to-end link bandwidth, $b$, disk read speed, $v_{read}$ at the source, or disk write speed, $v_{write}$ at the destination:

\begin{equation}
th_{max} \leqslant \textrm{min} \{b,v_{write},v_{read} \}
\end{equation}

For memory to memory transfers, $th_{max}$ is bounded by memory read, $m_{read}$
and write $m_{write}$ speed. 

\begin{equation}
th_{max} \leqslant \textrm{min} \{b,m_{write},m_{read} \}
\end{equation}

%\end{assumption}

%\begin{assumption}\label{as:rdma-agnostic}
Our model is agnostic to zero copy techniques used in Remote Direct Memory Access (RDMA) based transfer.  OS bypass might boost throughput when used with our model. %\end{assumption}

%\begin{assumption}\label{as:filesystem-agnostic}
Our model is for application-level optimization of the network data transfer protocols and it is agnostic of the underlying file systems. Due to the use of concurrency and parallelism, it would provide superior performance when parallel file systems are used at the end nodes.  
%
Performance degradation due to hardware misconfiguration, storage access delay, and intermediate network device bottlenecks could limit the achievable throughput. Eliminating such bottlenecks might increase the limit of achievable throughput.
%\end{assumption} 

%\begin{assumption}\label{as:link-failure}
For any kinds of link failure, the corresponding lower layers in the network stack make routing decisions for alternate links. Our model adapts with any such abrupt change in network by issuing new sets of parameters. In case of complete disconnection, transfer resumes until connection is recovered.    
%\end{assumption} 
\end{comment}

\begin{comment}
To understand the concept we need to discuss about the dataset that we have created. We performed 158,045 disk-to-disk transfer requests between XSEDE~\cite{XSEDE} nodes, in our local DIDCLab~\cite{DIDCLAB} testbed, and between our local testbed and the XSEDE nodes. Each request contains 8 to 1000 file transfers and the file sizes varied from 256KB to 3GB. This implies that more than 70 Million individual file transfers were performed  and monitored over six weeks to test and validate our model. An extensive 418 TB of data were transferred during the experiment. The GridFTP parameters -- pipelining, parallelism and concurrency levels were varied from 1 to 32 in the experiments. Among these parameters, concurrency has the most significant effect on utilizing the bandwidth and it provides enough distinct data to extract statistically viable optimization parameters for a given type of file transfers.  

The dataset contains $n$ entries. We can define our dataset as $D = \{ I_{1},I_{2},\ldots,I_{n}\}$. Each specific transfer $I_{i} , (1\leq i\leq n)$ consist of four components: (i) file transfer parameters $F_{i}$; (ii) network parameters $Nt_{i}$; (iii) throughput optimization parameters $Pm_{i}$; (iv) and achieved throughput $t_{i}$. We can define $I_{i} = \{F_{i},Nt_{i},Pm_{i},Th_{i}\}$. The file transfer parameter $ F_{i} = \{f_{i},n_{i}\}$, where $f_{i}$ is the average file size and $n_{i}$ is number of files. Similarly, the network parameter $N_{i} = \{b_{i},rtt_{i},bf_{i}\}$, where  $b_{i}$ is bandwidth of the network, $rtt_{i}$ is the round trip time, and $bf_{i}$ is the end system buffer-size. The optimization parameters $Pm_{i} = \{p_{i},cc_{i},pp_{i}\}$, where $p_{i}$ is parallelism level, $cc_{i}$ is concurrency level, and $p_{i}$ is the pipelining level. Now we can redefine entries of transfer history $I_{i}$ as 
\begin{equation}
I_{i} = \{f_{i},n_{i},b_{i},rtt_{i},bf_{i},p_{i},cc_{i},pp_{i},th_{i}\}
\end{equation}
 
A file transfer request $Req_{i}$ consist of file parameters and network characteristics which can be defined as
\begin{equation}
Req_{i} = \{F_{i},Nt_{i}\}
\end{equation}
 
Our goal is to find the best parameter combination $Pm_{i}^{''}$ that ensures maximum achievable throughput $t_{i}^{''}$. 
For each  $R_{i}$ , we varied $p, cc$ and $pp$ such that $p \;\epsilon \;\{p_{i1},p_{i2},\ldots,p_{ik}\}$,$\:$ $cc \;\epsilon \;\{cc_{i1},cc_{i2},\ldots,cc_{ik}\}$ and $pp \; \epsilon \;\{pp_{i1},pp_{i2},\ldots,pp_{ik}\}$ according to the following equations:

\begin{align}
p_{ik} = p_{ik-1}*2  \\
cc_{ik} = cc_{ik-1}*2 \\
pp_{ik} = pp_{ik-1}*2  
\end{align}

where $i \hspace{1mm}\epsilon \hspace{1mm} \{1,2,\ldots,n\}$ , $n$ is the number of transfer entries and $k$ is the level of variation in optimization parameters. So for each request $R_{i}$, the dataset has $k^{3}$ number of parameter combinations. We have used $k = 6$  in our dataset. Two transfer requests $Req_i$ and $Req_j$ with same parameters that run in different time of the day, might produce different throughput due to dynamic network condition and background traffic. Requests were scheduled across multiple days in peak and off-peak hours randomly. Repeated requests were performed at least a day apart. The experiment is performed continuously over six weeks to cover all off-peak and high-peak times. Each request Recorded throughput values for each settings $I_{i}$ can be   
\begin{equation}
th_i = \{t_{i1}, t_{i2},\ldots,t_{iq}\}
\end{equation}

From these $q$ samples we can compute statistically stable throughput value for that settings.
\end{comment}

==> section-dynamictuning.tex <==



This module is initiated when a user starts a data transfer request. Adaptive sampling is dependent on online measurements of network characteristics. It is essential to assess the dynamic nature of the network that is helpful to find the optimal parameter settings. A sample transfer could be performed to see how much throughput it can achieve. However, a single sample transfer could be error prone and might not provide clear direction towards the optimal solution. Our algorithm adapts as it performs sample transfers by taking guidance from offline surface information. This approach can provide faster convergence. An overview of the module is presented in Algorithm (\ref{algo:onlinesampling}).  Online module queries the offline analysis module with network and dataset characteristics.  Offline module finds the closest cluster and returns the throughput surfaces along with associated external load intensity information and suitable sampling region for each surface. 

%In a shared environment, there could be many transfers those are not explicitly logged, however, those unknown transfers could have an impact on the achievable throughput as well.  We define the impact of those uncharted transfers as external load intensity, $I_{s}$ and model is with a simple heuristics:

%\begin{equation}
%I_s = \dfrac{bw - th_{out} }{bw}
%\end{equation}

The online module sorts the surfaces in descending order based on external load intensity value (Lines 17-18).  
Adaptive sampling module takes the dataset that is needed to be transferred and starts performing sample transfers from the dataset. To perform the first sample transfer, the algorithm chooses the surface with median load intensity, $f_{median}$, and performs the transfer with: 

\begin{equation}
\theta_{s,median} = \{p,cc,pp\} = \mathrm{argmax}(f_{s,median})
\end{equation}

%%% Adaptive Sampling Algorithm:
\IncMargin{1em}
\begin{algorithm}[t]
	\SetKw{in}{in}
	\SetKwData{Left}{left}\SetKwData{This}{this}
    \SetKwData{Up}{up}\SetKwData{Log}{Log}
    \SetKwData{ismedian}{$e_{s,median}$}\SetKwFunction{Median}{Median}
    \SetKwFunction{Union}{Union}
    \SetKwFunction{FindCompress}{FindCompress}
    \SetKwFunction{FindClosestSurface}{FindClosestSurface}
    \SetKwFunction{GetOptimalParam}{GetOptimalParam}
    \SetKwFunction{DataTransfer}{DataTransfer}
    \SetKwFunction{AdaptiveSampling}{AdaptiveSampling}
    \SetKwFunction{append}{append}
    \SetKwFunction{remove}{remove}
    \SetKwFunction{QueryDB}{QueryDB}
    \SetKwFunction{Sort}{Sort}
    \SetKwFunction{GetSamples}{GetSamples}
	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
    \tcp{Source, $EP_{s}$, Destination, $EP_{d}$, Round trip time, $rtt$, Bandwidth, $bw$}
	\Input{Data arguments, $data\_args = \{Dataset , avg\_file\_size, num\_files\}$,
           network arguments, $net\_args = \{EP_s, EP_d, rtt, bw\}$,  
           transfer node arguments, $node\_args = \{num\_nodes,cores, memory, NIC\_speed \}$}
	\Output{Optimal transfer rate, $th_{opt}$}
	\BlankLine
	%\emph{special treatment of the first line}\;
    \SetKwProg{proc}{procedure}{}{}
    \proc{\AdaptiveSampling{$F_s$, $R_s$, $I_s$} }{
    	$D_{s}$ $\leftarrow$ \GetSamples{$Dataset$}  \\
        
    	\ismedian  $\leftarrow$ \Median{$I_s$} \\
        $f_{s,median}$ $\leftarrow$ $F_{s}[e_{s,median}]$ \\
        $\theta_{s,median}$, $th_{hist}$ $\leftarrow$ \GetOptimalParam{$f_{s,median}$} \\
        $th_{cur}$ $\leftarrow$ \DataTransfer{$D_{s,1}$,$p_{s,median}$} \\
        \Log.\append{$net\_args$, $D_{s,i}$,$p_{s,median}$,$th_{cur}$} \\
        $D_{s}$.\remove{$D_{s,1}$} \\
        \For{$D_{s,i}$ \in $D_s$ } {
              \If{$th_{cur}$ $\neq$ $th_{hist}.confidence\_bound$} { 
                   $f_{s,cur}$ $\leftarrow$ \FindClosestSurface{$th_cur$} \\
                   $p_{s,cur}$, $th_{hist}$ $\leftarrow$ \GetOptimalParam{$f_{s,curr}$} \\
                   $th_{cur}$ $\leftarrow$ \DataTransfer{$D_{s,i}$,$p_{s,cur}$} \\
                   \Log.\append{$net\_args$, $D_{s,i}$,$p_{s,cur}$,$th_{cur}$}
              }
        }
    }
    
    $F_s$, $R_s$, $I_s$ $\leftarrow$ \QueryDB{$data\_args$,$net\_args$} \\
	$F{'}_{s}$ $\leftarrow$ \Sort{$F_s$,$I_s$} \\
    \tcp{Set of surfaces, $F_{s}$, Sampling region, $R_{s,k}$, Load intensity, $I_s$ }
	\AdaptiveSampling{$F^{'}_{s}$, $R_{s,k}$, $I_s$}
\caption{Online Sampling}
\label{algo:onlinesampling}
\end{algorithm}\DecMargin{1em}



which is already precomputed during offline analysis and can be found in the sampling region. Achieved throughput value for the transfer is recorded (Lines 2-6). If the achieved throughput is inside the surface confidence bound at point $\theta_s,median$, then the algorithm continues to transfer rest of the data set chunk by chunk. However, if the achieved throughput is outside the confidence bound, that means the current surface is not representing the external load of the network. If achieved throughput is higher than the surface maxima, that means current network load is lighter than the load associated with the surface. Therefore, the algorithm searches the surfaces with lower load intensity tags and find the closest one and perform second sample transfer with parameters of newly found surface maxima. In this way, the algorithm can get rid of half the surfaces at each transfer. At the point of convergence, our algorithm takes the rest of the dataset and starts the transfer process. Changing parameters in real-time is expensive. For example, if a $cc$ value changes from 2 to 4, this algorithm has to open two more server processes and initialize resources. These new processes have to go through TCP's slow start phase as well. Therefore, the algorithm tries to minimize the initial sampling transfers by the adaptive approach. For very large-scale transfers, when data transfer happens for a long period of time, external traffic could change during the transfer. If the algorithm detects such deviation, it uses most recently achieved throughput value to choose the suitable surface and changes the transfer parameters.   











==> section-offlineoptimization.tex <==
%Why historical log is necessary?
%Why offline analysis is necessary?


%Individual parameter impact on throughput is well understood. However, the joint impact along with different network conditions are not accurate and sometimes complex to understand. Analyzing the historical log can provide helpful guidance towards near-optimal solution. 

%A natural solution is to use an regression or interpolation model to accurately capture the relationship among network conditions and contending transfers. 

%Show a graph with cubic interpolation. (detail later)

%Underlying TCP provides per flow fairness. How to provide individual user fairness, when multiple channels are involved.

%Propose a centralized solution

%Efficient allocation of resources to the transfer processes. Sub optimal allocation reduce the transfer efficiency. (figure)

%Network condition measure (Non intrusive)- RTT, Queuing delay, known contending transfers, performance of streams, unknown contending transfers.


%Our model consists of two phases: \textit{(i)} offline knowledge discovery \textit{(ii)} online adaptive sampling. The offline analysis module is an additive model. That means when new logs are generated for a certain period of time, we do not need to combine them with previous logs and perform analysis on the entire log \textit{(old log + new log)} from scratch. Users do not need to perform offline analysis during each transfer. Data transfer logs can be collected for a certain period of time and then the additive offline analysis can be performed on those new logs only. For services like Globus, historical logs can be analyzed by a dedicated server and results can be shared by the users. When a user starts data transfer process, the system initiates online adaptive sampling. Adaptive sampling module queries the results of the offline analysis module which can be answered in constant time. The adaptive sampling guided by offline analysis provides faster convergence towards near-optimal throughput. 

%\subsection{Offline Analysis}
%\label{subsec:Offlineanalysis}
Offline analysis collects useful information from the historical logs so that those information can be used by the online module to converge faster. Offline analysis consists of five phases: \textit{(i)} clustering logs in hierarchy; \textit{(ii)} surface construction; \textit{(iii)} finding maximal parameter setting; \textit{(iv)} accounting for known contending transfers; and \textit{(v)}identifying suitable sampling regions. 

\subsection{Clustering logs}
\label{sub:clusteringlogs}
Historical data transfer logs contain information about the verity of transfers performed by the users. Therefore, a natural approach would be cluster the logs based on different matrices. Assuming that we have a historical log, $L$ of $n_{log}$ log entries, We can define our clustering problem as $(L,m)$, where $m$ is the number of target clusters. The clusters of the historical logs are $C = \{ C_{1},...,C_{m}\}$, where $\{n_{1},...,n_{m}\}$ denote the sizes of the corresponding clusters. We consider a pairwise distance function, $\it{d}(x,x^\prime)$ where $x,x^\prime \in L$. We have tested clustering algorithm for different pair-wise distance functions. For clustering, we have tested two well-known approaches: (1) K-means++~\cite{kmeans++}; (2) Hierarchical Agglomerative  Clustering (HAC) with Unweighted Pair Group Method with Arithmetic Mean (UPGMA)~\cite{upgma_clustering}. K-means clustering algorithm suffers from initial centroid selection, and wrong initialization could lead to wrong clustering decision. However, K-means++ provides a theoretical guarantee to find a solution that is $O(log\ m)$ competitive to the optimal K-means solution. For HAC, distance between two clusters $C_{i}$ and $C_{j}$ is defined as $D(C_{i},C_{j})$ in Equation (\ref{eq:UPGMAdistance}):

\begin{equation}
\label{eq:UPGMAdistance}
D(C_{i},C_{j}) = d(c_i,c_j) = \sqrt[]{(c_i - c_j)^{2}}
\end{equation}

Where $c_i$ and $c_j$ are the corresponding cluster centroid of $C_i$ and $C_j$. HAC computes proximity matrix for the initial clusters and combines two clusters with minimum distance $D(C_i,C_j)$. Then, it updates the rows and columns of proximity matrix with new clusters and fills out the matrix with new $D(C_i,C_j)$. This process is repeated until all clusters are merged into a single cluster. 

Clustering accuracy depends on the appropriate number of clusters $k$. In this work, we have used Calinski and Harabasz index (CH index) to identify the appropriate number of clusters. CH index can be computed as:
\begin{equation}
CH(m) = \dfrac{\Phi_{inter}(m)/(m-1)}{\Phi_{inter}(m)/(n-m)}
\end{equation}
Where $\Phi_{inter}$ is the ``between-cluster" variation and $\Phi_{intra}$ is the ``within-cluster"" variation. Both can be defined as the sum of Euclidean distance as bellow:

\begin{equation}
 \Phi_{inter}(m) = \sum^{m}_{i=1} \sum_{x \in c_i} (x - c_i)^2
\end{equation}

\begin{equation}
 \Phi_{intra}(m) = \sum^{m}_{i=1} n_k(\bar{C_k} - \bar{x})^2
\end{equation}
Where $\bar{C_k}$ is the mean of points in cluster $k$ and $\bar{x}$ is the overall mean. Largest $CH(m)$ score is preferable. 




\subsubsection{Surface Construction}
\label{subsubsec:surfaceconstruction}
Achievable throughput for a given cluster $C_{i}$ can be modeled as a polynomial surface which depends on the protocol tuning parameters. We have tried three models to see how accurate those can capture the throughput behavior. The models are: (1) quadratic regression; (2) cubic regression; and (3) piecewise cubic interpolation. 

\begin{comment}
\textbf{\textit{(i) Quadratic regression.}} A quadratic surface can be represented as: 
\begin{equation}
f(p,cc,pp) = t_{1}p^{2} + t_{2}cc^{2} + t_{3}pp^{2} +...+ t_{k-2}cc + t_{k-1}pp + t_{k} 
\end{equation}
Where $t_{1}, t_{2},...,t_{k}$ are the parameters of the surface which can be estimated by minimizing the least-squared error. 
\begin{equation}
\underset{ t_{1},...,t_{k} }{\mathrm{min}} \sum_{i = 1}^{n} [f(p_i,cc_i,pp_i) - th_{i}]^2
\end{equation}

However, it under-fits the historical log severely. One of the good side of this modeling is that it provides a bitonic surface which is easy to explore. 

\textbf{\textit{(ii) Cubic regression.}} A multivariate cubic surface can be represented as:
\begin{equation}
f(p,cc,pp) = t_{1}p^{3} + t_{2}cc^{3} + t_{3}pp^{3} + ...+ t_{k^\prime-1}pp + t_{k^\prime} 
\end{equation}
Corresponding least squared minimization problem can be defined as:
\begin{equation}
\underset{ t_{1},...,t_{k^\prime} }{\mathrm{min}} \sum_{i = 1}^{n} [f(p_i,cc_i,pp_i) - th_{i}]^2\\
\quad \mathrm{s.t.} \quad f(p,cc,pp) > 0
\end{equation}
This model also suffers from under-fitting the cluster data from historical logs. One way to resolve this under-fitting problem is by introducing piece-wise polynomials between the data samples with a guarantee of smoothness up to second derivatives.

%Pipelining parameter acts differently 
\end{comment}

\textbf{\textit{ Piecewise cubic spline interpolation.}} We model throughput with cubic spline surface interpolation \cite{kincaid2009numerical}. Before introducing the interpolation method, we should explain the relationship among the parameters briefly. Concurrency and pipelining are responsible for a total number of data streams during the transfer, whereas, pipelining is responsible for removing the delay imposed by small files. Due to their difference in characteristic, we model them separately. At first, we construct a $2$-dimension cubic spline interpolation for $g(pp) = th$. Given a group of discrete points in $2$-dimension space $\{(pp_i,th_i)\}, i = 0,...,N$, the cubic spline interpolation is to construct the interpolant $g(pp) = th$ by using piecewise cubic polynomial $g_i(pp)$ to connect between the consecutive pair of points $(pp_i,th_i)$ and $(pp_{i+1},th_{i+1})$. The coefficients of cubic polynomials are constrained to guarantee the smoothness of the reconstructed curve. This is implemented by controlling the second derivatives since each piecewise relaxed cubic polynomial $g_i$ has zero second derivative at the endpoints. Now we can define each cubic polynomial piece as:  
%Assuming there is no reason to bend the curve at the endpoints, a relaxed cubic polynomial has zero second derivative at the endpoints. The corresponding mathematical 
%We can approximate $f(x)$ with piece-wise cubic polynomial, 
%The whole curve $y = g(x)$ can be e
\begin{equation}
g_i(pp) = c_{i,0} + c_{i,1}pp + c_{i,2}pp^2 + c_{i,3}pp^3,\forall pp \in [pp_i,pp_{i+1}].
\end{equation}

Periodic boundaries can be assumed as $g(pp_{i+1}) = g(pp_i)$. Coefficients $c_{i,j}$, where $j = 1,2,3$, of piece-wise polynomial $g_i(pp)$ contains $4(N-1)$ unknowns. We can have:
\begin{equation}
g_i(pp_i) = th_i, \quad i = 1,...,N
\end{equation}
Hence, the $N$ continuity constraints of $g(pp)$ are as:
\begin{equation} \label{eq:constraint2}
g_{i-1}(pp_i) = th_i = g_{i}(pp_i), \quad i = 2,...,N.
\end{equation}
We can get $(N-2)$ constraints from Equation (\ref{eq:constraint2}) as well. We can impose additional continuity constraints up to second derivatives. 
\begin{equation} \label{eq:constraint3}
\dfrac{d^2 g_{i-1}}{d^2 pp} (pp_i) = \dfrac{d^2 g_{i}}{d^2 pp} (pp_i), \quad i = 2,...,N
\end{equation}
We can get $2(N-2)$ constraints from Equation (\ref{eq:constraint3}). The boundary condition for relaxed spline could be written as:

\begin{equation} \label{eq:constraint4}
\dfrac{d^2 g}{d^2 pp} (pp_1) =  \dfrac{d^2 g}{d^2 pp} (pp_n) = 0
\end{equation}

So we have $N + (N-2) + 2(N-2) +2 = 4(N-1)$ constraints in hand. The coefficients can be computed by solving the system of linear equations. This example is extended to generate surface with two independent variables.

Then, we model throughput as a piece-wise cubic spline surface. It can be done by extending the $2$-dimension cubic interpolation scheme presented above  to model the function of throughput. A short overview is given below:
We first fix the value of $pp$.
The throughput $f(p,pp,cc)$ then becomes $f_{pp}(p,cc)$
which is a surface in $\Psi^2 \times \mathbb{R}$. Where $\Psi$ domain of parameters $\{cc, p, pp\}$.  
Data points can be represented as
$P = \{ (p_{i},cc_{j},th_{i,j}) | i = 1,2,\ldots,N, j = 1,2,\dots,M, (x_i,y_j) \in G \}$,
where $G$ is an $N \times M$ rectangle grid,
and each $(p_{i},cc_{j})$ denotes the grid point at $i$-th row and $j$-th column. The piecewise cubic interpolation method will construct
an interpolated cubic function $f_{r(i,j)}(p,cc)$
for each rectangle $r(i,j)$ from the grid $G$,
where $r(i,j)$ rectangle can be defined by $[p_i, p_{i+1}] \times [cc_j, cc_{j+1}]$.
%
$f_{r(i,j)}(p,cc)$ should fit the $th$-values of $P$ at the vertices of $r(i,j)$, \emph{i.e.}

\begin{gather*} 
f_{r(i,j)}(p_i,cc_j) = th_{i,j} \\
f_{r(i,j)}(p_{i+1},cc_j) = th_{i+1,j} \\
f_{r(i,j)}(p_i,cc_{j+1}) = th_{i,j+1} \\
f_{r(i,j)}(p_{i+1},cc_{j+1}) = th_{i+1,j+1} \\
\end{gather*} 

The interpolated cubic functions should also maintain smoothness at grid points. The continuity constraints are computed as an extension of   Equation (\ref{eq:constraint3}) and  (\ref{eq:constraint4}). 

Formally, this means that there exist numbers
$\Omega_{1}(i,j), \Omega_{2}(i,j), \Omega_{1,2}(i,j)$ for each $i = 1,2,\ldots,N, j = 1,2,\dots,M$,
such that for each $rect(i,j)$, and each vertex $(p_{i'},cc_{j'})$ of $rect(i,j)$,
\[
(\partial f_{r(i,j)}(p_i,cc_j) / \partial p)|_{p_{i'},cc_{j'}} = D_{1}(i',j')
\]
\[
(\partial f_{r(i,j)}(p_i,cc_j) / \partial cc)|_{p_{i'},cc_{j'}} = D_{2}(i',j')
\]
\[
(\partial f_{r(i,j)}(p_i,cc_j) / \partial p \partial cc)|_{p_{i'},cc_{j'}} = D_{1,2}(i',j')
\]

After solving the  constraints (which is a linear system),
all the functions $f_{rect(i,j)}(x,y)$ where $i = 1,2,\ldots,N-1, j = 1,2,\dots,M-1$
form a piecewise smooth function which fixes data point set $P$.
Figure \ref{fig:3diinterpolation} shows the constructed piece-wise cubic surfaces of throughput for different $cc$ and $p$ values. We can see from the graph surfaces for small files are more complex than the medium and large file. 
%Figure \ref{fig:ppCurve} shows interpolated curve of throughput for different $pp$ values.
Figure \ref{fig:surface_accuracy}(b) shows the accuracy of different surface construction models. It can be seen that piece-wise cubic spline outperforms all other models and achieves almost 85\% accuracy. 

%\end{comment}

\begin{comment}
\vspace{5mm}
(1) New Version:
\vspace{5mm}

Therefore, we apply an piecewise cubic interpolation scheme to
model the function of the throughput.
In the following, we first fix the value of $pp$.
The throughput $f(p,pp,cc)$ then becomes $f_{pp}(p,cc)$
which is a surface in $\mathbb{R}^3$.
To reconstruct the surface from the throughput log data
which contains a number of values of $p_i$,
$cc_i$ and the corresponding throughput $f_{pp}(p_i,cc_i)$,
we use the method of piecewise cubic interpolation.

Here we give a brief introduction to the method.
Given a set of $\mathbb{R}^3$ data points denoted by
$P = \{ (x_{i},y_{j},z_{i,j}) | i = 1,2,\ldots,N, j = 1,2,\dots,M, (x_i,y_j) \in G \}$,
where $G$ is an $N \times M$ rectangle grid,
and each $(x_{i},y_{j})$ denotes the grid point at $i$-th row and $j$-th column,
the piecewise cubic interpolation method will construct
a interpolate cubic function $f_{rect(i,j)}(x,y)$
for each rectangle $rect(i,j)$ from the grid $G$,
where $rect(i,j)$ denotes the rectangle defined by $[x_i, x_{i+1}] \times [y_j, y_{j+1}]$.

$f_{rect(i,j)}(x,y)$ should fit the $z$-values of $P$ at the vertices of $rect(i,j)$, \emph{i.e.}
\[
f_{rect(i,j)}(x_i,y_j) = z_{i,j}
\]
\[
f_{rect(i,j)}(x_{i+1},y_j) = z_{i+1,j}
\]
\[
f_{rect(i,j)}(x_i,y_{j+1}) = z_{i,j+1}
\]
\[
f_{rect(i,j)}(x_{i+1},y_{j+1}) = z_{i+1,j+1}
\]
The interpolate cubic functions should also maintain smoothness at grid points.
Formally, this means that there exist numbers
$D_{1}(i,j), D_{2}(i,j), D_{1,2}(i,j)$ for each $i = 1,2,\ldots,N, j = 1,2,\dots,M$,
such that for each $rect(i,j)$, and each vertex $(x_{i'},y_{j'})$ of $rect(i,j)$,
\[
(\partial f_{rect(i,j)}(x,y) / \partial x)|_{x_{i'},y_{j'}} = D_{1}(i',j')
\]
\[
(\partial f_{rect(i,j)}(x,y) / \partial y)|_{x_{i'},y_{j'}} = D_{2}(i',j')
\]
\[
(\partial f_{rect(i,j)}(x,y) / \partial x \partial y)|_{x_{i'},y_{j'}} = D_{1,2}(i',j')
\]
As a result of solving the above constrains(which is indeed a linear system),
all the functions $f_{rect(i,j)}(x,y)$, $i = 1,2,\ldots,N-1, j = 1,2,\dots,M-1$
form a piecewise smooth function which fixes data point set $P$.

We perform the above method to obtain fitting function $f_{pp}(p_i,cc_i)$ for throughput when $pp$ is fixed.
We perform interpolation for each possible value of $pp$ to have a complete picture of throughput
in terms of $p$, $pp$ and $cc$.
\end{comment}


% \vspace{5mm}
% (2)Previous Version:
% \vspace{5mm}



% \begin{figure}
% 	\begin{subfig}[H]
%     	\includegraphics[width=40mm]{figures/Guassian_fit.png}
% 		\caption{(a)}
% 	\end{subfigure}
% 	\quad
% 	\begin{subfig}[H]
% \includegraphics[width=40mm]{figures/surface_fitting_accuracy.png}
% 		\caption{(b)}
% 	\end{subfigure}
% \caption{Distribution of throughput values under similar external loads and Accuracy of different surface construction methods}
% \end{figure}







Data transfer requests within the same cluster $C_{i}$ with the same protocol parameter values might have a deviation from one another due to measurement errors and many other network uncertainties such as different packet route in the network layer and minor queuing delay. %Figure~\ref{fig:surface_accuracy}(a) shows that this deviation follows the Gaussian distribution.
We define those data points with the same protocol parameter entries as $\omega$. To model this deviation, we have used a Gaussian confidence region around each constructed surface. The probability density function of a Gaussian distribution is: 

\begin{eqnarray}
&& p(\omega;\mu,\sigma) = \dfrac{1}{\sqrt{2\pi\sigma^2}}e^{-\dfrac{(\omega-\mu)^2}{2\sigma^2}}, \label{eq:confidence}\\
&& \mu = \frac{1}{N}\sum_{i=1}^N th_i, \label{eq:confidence:mean}\\
&& \delta = \sqrt{\frac{1}{N}\sum_{i=1}^N(th_i-\mu)^2}, \label{eq:confidence:var}
\end{eqnarray}
where $\mu$ is the mean and $\sigma$ is the standard deviation of the data distribution. Figure \ref{fig:surface_accuracy}(a) shows the data model for the Gaussian distribution.

\subsubsection{Finding Maximal Parameters}
\label{subsubsec:findingmaximalparams}
Very high protocol parameter values might overburden the system. For this reason, many systems set upper bound on those parameters. Therefore, the parameter search space has a bounded integer domain. Assuming $\beta$ is the upper bound of the parameters, cubic spline surface functions can be expressed as $f_i: \Psi^{3} \Rightarrow \mathbb{R}^{+}$, where $\Psi = \{1,2,..,\beta\}$. To find the surface maxima, we need to generate all local maxima of $F = \{f_1,...,f_p\}$. This is achieved by performing the second partial derivative test on each $f_k$ \cite{kincaid2009numerical}. The main idea is presented below. 

First, we calculate the Hessian matrix of $f_k$ as:%have used analytical approach which is efficient and accurate. First, we compute the Jacobian matrix of spline function set ${f_1,...,f_p}$ with respect to $(p, cc, pp)$. 
\begin{equation}
\label{eq:Hessian_fk}
H_k = J(\bigtriangledown f_k) =\left[ {\begin{array}{*{20}c}
   \dfrac{\partial^2 f_k}{\partial p^2} & \dfrac{\partial^2 f_k}{\partial p\ \partial cc} & \dfrac{\partial^2 f_k}{\partial p\ \partial pp}  \\
   ... & ... & ... \\
\dfrac{\partial^2 f_k}{\partial pp\ \partial p} & \dfrac{\partial^2 f_k}{\partial pp\ \partial cc} & \dfrac{\partial^2 f_k}{\partial pp^2}  \\  
 \end{array} } \right],
\end{equation}
where $J$ stands for the Jacobian matrix:
\begin{equation}
J(F) = \left[ {\begin{array}{*{20}c}
   \dfrac{\partial f_1}{\partial p} & \dfrac{\partial f_1}{\partial cc} & \dfrac{\partial f_1}{\partial pp}  \\
   ... & ... & ... \\
\dfrac{\partial f_p}{\partial p} & \dfrac{\partial f_p}{\partial cc} & \dfrac{\partial f_p}{\partial pp}  \\  
 \end{array} } \right]
\end{equation}
% For a spline function $f_k$, we perform a second partial derivative test using its Hessian matrix.%if a local maxima exist at point $(x,y,z)$ then Jacobian matrix will be zero at $(x,y,z)$. We can mark $(x,y,z)$ as a critical point. Then we have to compute the Hessian matrix at point $(x,y,z)$. 

% \begin{equation}
% H_k = J(\bigtriangledown f_k) \left[ {\begin{array}{*{20}c}
%    \dfrac{\partial^2 f_k}{\partial p^2} & \dfrac{\partial^2 f_k}{\partial p\ \partial cc} & \dfrac{\partial^2 f}{\partial p\ \partial pp}  \\
%    ... & ... & ... \\
% \dfrac{\partial^2 f}{\partial pp\ \partial p} & \dfrac{\partial^2 f}{\partial pp\ \partial cc} & \dfrac{\partial^2 f}{\partial pp^2}  \\  
%  \end{array} } \right]
% \end{equation}


\begin{comment}
\begin{figure}[t]
\centering
\includegraphics[keepaspectratio=true,angle=0, height= 40mm]{figures/pp_curve_fig.eps}
\vspace{-3mm}
\caption{Piece-wise cubic interpolation of throughput over pipelining. } 
\label{fig:ppCurve}
\end{figure}
\end{comment}


\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.2\textwidth}
    	\centering
        \hspace{-1.2cm}
        \includegraphics[keepaspectratio=true,width=45mm]{figures/Guassian_fit.png}
        \caption{}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.2\textwidth}
    \centering
        \includegraphics[keepaspectratio=true,width=44mm]{figures/surface_fitting_accuracy.png}
        \caption{}
    \end{subfigure}
    \caption{(a) Distribution of throughput values under similar external loads; b) Accuracy of different surface construction methods.}
    \label{fig:surface_accuracy}
\end{figure}


Then we obtain the coordinates of all local maxima in $f_k$ by calculating the corresponding $\{p,pp,cc\}$'s such that $H_k(p,pp,cc)$ is negative definite. Hence, the set of local maxima of $f_k$ is obtained. Finally, the surface maxima is generated by taking the maximum among all local maxima sets of $F$. 

% The complexity of calculating surface maxima is $O(p)$. It is because, for each $f_k$, we only need constant numbers of operations in calculating its local-maxima set. Actually, $H_k$ is always a $3$-by-$3$ matrix, due to $(p,pp,cc)\in \mathcal{R}^3$. And there are finite numbers of stationary points for a cubic polynomial $f_k$ in a bounded domain \cite{kincaid2009numerical}. Thus, only constant numbers of operations is needed in performing the negative-definiteness check. Therefore complexity $O(1)$ is required for solving the set of local maxima of $f_k$. 
% \begin{equation}
% \textrm{When} \quad \mathrm{Det}(H) > 0, \quad \textrm{and} \quad \dfrac{\partial^2 f}{\partial p^2} < 0
% \end{equation}

%If the condition satisfies then the point $(x,y,z)$ is the local maxima. We can find all the local maxima in the bounded region and take the maximum one as surface maxima. 



\subsubsection{Accounting for Known Contending Transfers}
\label{subsubsec:accountingforcontendingtransfers}
Underlying TCP protocol tries to provide a fair share of bandwidth to all data streams concurrently transferring data. Assume we are analyzing a data transfer log entry $t_{p}$, any contending transfer in source or destination can have an impact on transfer request $t_{p}$. Known contending transfers are the ones present in the historical log and can be classified into five types:

\textbf{\textit{(i) Same source and destination.}} Contending transfers with the same source and destination is denoted as $t_{c}$. In Figure~\ref{fig:srcDst},  $t_c$ has an aggregate transfer rate $r_{c}$ and parameter settings $param\_t_{c}$.

\textbf{\textit{(ii) Source outgoing.}} Outgoing transfers from the source node of $t_{p}$ to different destinations. We defined those transfers as $t^{src}_{out}$ with aggregate transfer rate $r^{src}_{out}$ and parameter settings $param\_t^{src}_{out}$. 

\textbf{\textit{(iii) Source incoming.}} Incoming transfers to the source $t^{src}_{in}$ with aggregate transfer rate $r^{src}_{in}$ and parameters settings $param\_t^{src}_{in}$.

\textbf{\textit{(iv) Destination outgoing.}} Outgoing transfers from the destination node of $t_{p}$ with different destinations. We defined those transfers as $t^{dst}_{out}$ with aggregate transfer rate $r^{dst}_{out}$ and parameter settings $param\_t^{dst}_{out}$. 

\textbf{\textit{(v) Destination incoming.}} Incoming transfers to the destination of $t_p$ named as $t^{dst}_{in}$ with aggregate transfer rate $r^{dst}_{in}$ and parameter settings $param\_t^{dst}_{in}$.

Figure \ref{fig:srcDst} describes the known contending transfers in both source and destination nodes. In a shared environment, there could be many transfers those are not explicitly logged, however, those unknown transfers could have an impact on the achievable throughput as well.  We can define the impact of those uncharted transfers as external load intensity, $I_{s}$, and model it with a simple heuristics:

\begin{equation}
I_s = \dfrac{bw - th_{out} }{bw}
\end{equation}

\begin{figure}[t]
\centering
\includegraphics[keepaspectratio=true,angle=0,width=85mm]{figures/Dst.pdf}
\vspace{-3mm}
\caption{Different types of known contending transfers.} \label{fig:srcDst}
\end{figure}

\subsubsection{Identifying Suitable Sampling Regions}
\label{subsubsec:unknownload}
Identifying the suitable sampling region is a crucial phase that helps online adaptive sampling module to converge faster. %From the previous phases, we know the cluster $C_{i,j,k}$ contains the throughput surfaces with different load intensities.
%Those surfaces interpolate throughput inside the bounded domains of the parameters. However, 
However, not all the regions on a surface are interesting. Many parameter coordinates of a surface are suboptimal. We are interested in regions which have a better possibility of achieving high throughput. The regions containing distinguishable characteristics of the surfaces and containing the local maxima of those surfaces are more compelling. Exploring those regions could lead to a near-optimal solution much faster. Assume the cluster $C_{i}$ contains $\eta$ number of the surfaces that can be written as $S = {f_{1}, ... f_{\eta}}$. Now, we can extract the neighborhood with a predefined radius $r_d$ that contains maxima for all the surfaces in $S$. Assume the set $R_m$ contains all those neighborhood of maxima. We are also interested in regions where surfaces are clearly distinguishable. The goal is to find the regions where surfaces are maximally distant from one another. This problem can be formulated as a max-min problem. Selection can be done by taking the maximum of all pair shortest distance between the surfaces. To achieve that we perform uniform sampling $u = \{u_{1},...,u_{\gamma}\}$ from surface coordinate $(p,cc,pp)$  for surfaces in $S$. Therefore, $u$ could be written as: 

\begin{equation}
u = \{u_{1},...,u_{\gamma}\} =  \{(p_i,cc_i,pp_i)\}^{\gamma}_{i=1} 
\end{equation}
We define $\Delta^{min}_{u_i}$ as the minimum distance between any two pair of surfaces that can be expressed as: 
\begin{equation}
\label{eq:region_selection}
\forall u_{k} \in u, \quad \Delta^{min}_{u_k} = \underset{ \forall i,j \in \{1,...,\eta\} }{\mathrm{min}} |f_{i}(u_k) - f_{j}(u_{k})| \quad \textrm{where} \quad i \neq j
\end{equation}
 
 After sorting the list in descending order we choose, $\lambda$ $(1<\lambda < k)$, number of the initial samples from the sorted list.  
 Assume the set of points we get after solving the Equation (\ref{eq:region_selection}) is $R_c$. We define suitable sampling region as :
 \begin{equation}
R_s = R_m \cup R_c
\end{equation}
During online analysis, we will use the region in $R_s$ to perform the sample transfers.

%\vspace{5mm}

